Machine Learning for Mechanical Ventilation Control (Extended Abstract)

Mechanical ventilation is one of the most widely used therapies in the ICU. However, despite broad application from anaesthesia to COVID-related life support, many injurious challenges remain. We frame these as a control problem: ventilators must let air in and out of the patient's lungs according to a prescribed trajectory of airway pressure. Industry-standard controllers, based on the PID method, are neither optimal nor robust. Our data-driven approach learns to control an invasive ventilator by training on a simulator itself trained on data collected from the ventilator. This method outperforms popular reinforcement learning algorithms and even controls the physical ventilator more accurately and robustly than PID. These results underscore how effective data-driven methodologies can be for invasive ventilation and suggest that more general forms of ventilation (e.g., non-invasive, adaptive) may also be amenable.

==> ML4H 2021 Extended Abstract/defs.tex <==
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{xcolor}         % colors
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{times}
\usepackage{amsfonts}
\usepackage{mathtools, enumitem}
\usepackage{latexsym}
\usepackage{relsize}
\usepackage{mathrsfs, float}
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{xcolor}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{dsfont}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}

\newcommand{\softmax}{\text{softmax}}
\newcommand{\CH}{\text{CH}}
\newcommand{\F}{\mathcal{F}}
%\newcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\DeclareMathOperator{\Tr}{Tr}
\definecolor{PrincetonOrange}{HTML}{ff8f00}

% change these macros to different names.
\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}


\def\ltil{{{\tilde{\ell}}}}
\def\btalpha{{\bm{\tilde{\alpha}}}}
\def\balpha{{\bm{\alpha}}}
\def\talpha{{\tilde{\alpha}}}
\def\btbeta{{\bm{\tilde{\beta}}}}
\def\bbeta{{\bm{\beta}}}
\def\tbeta{{\tilde{\beta}}}
\def\btgamma{{\bm{\tilde{\gamma}}}}
\def\bgamma{{\bm{\gamma}}}
\def\tgamma{{\tilde{\gamma}}}


\def\mL{{\mathcal L}}

\def\X{{\mathcal X}}
\def\H{{\mathcal H}}
\def\Y{{\mathcal Y}}
\def\W{{\mathcal W}}
\def\R{{\mathbb R}}


% notation here
\newcommand{\ftil}{\tilde{f}}

\def\hestinv{\tilde{\nabla}^{-2}}
\def\hest{\tilde{\nabla}^{2}}
\def\hessinv{\nabla^{-2}}
\def\hess{\nabla^2}
\def\grad{\nabla}


% notation

\newcommand{\re}{{\text{Re}}}
\newcommand{\B}{B}
%\newcommand{\R}{\mathcal{R}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\cE}{\mathcal{E}}
\renewcommand{\sp}{\mathrm{span}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\cor}{\mathrm{cor}}
\newcommand{\sign}{\text{ } \mathrm{sign}}


\newcommand{\bzero}{\ensuremath{\mathbf 0}}
\newcommand{\y}{\ensuremath{\mathbf y}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\h}{\ensuremath{\mathbf h}}
\newcommand{\K}{\ensuremath{\mathcal K}}
\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\C{{\mathcal C}}

%\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
%\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\x{\mathbf{x}}
\def\y{\mathbf{y}}
\def\w{\mathbf{w}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
%\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bS{\mathbf{S}}
\def\bG{\mathbf{G}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}

\def\regret{\mbox{{Regret}}}

\def\ytil{\tilde{{y}}}
\def\yhat{\hat{{y}}}
\def\what{\hat{{w}}}
\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}



% comments, etc
\newcommand{\ignore}[1]{}
% for emails
\newcommand{\email}[1]{\texttt{#1}}



% repeated theorems

\newenvironment{repthm}[2][]{%
  \def\theoremauxref{\cref{#2}}
  \begin{theoremaux}[#1]
}{%
  \end{theoremaux}
}



% bold serif
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}

% operators
\DeclareMathOperator*{\err}{error}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\supp}{supp}
%\DeclareMathOperator*{\poly}{poly}
\let\Pr\relax
\DeclareMathOperator{\Pr}{\mathbb{P}}

% cases
\newcommand{\mycases}[4]{{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}}
\end{array}
\right. }}

\newcommand{\mythreecases}[6] {{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}} \\[1ex]
    {#5} & {\;\text{#6}}
\end{array}
\right. }}

% macros
\newcommand{\lr}[1]{\!\left(#1\right)\!}
\newcommand{\lrbig}[1]{\big(#1\big)}
\newcommand{\lrBig}[1]{\Big(#1\Big)}
\newcommand{\lrbra}[1]{\!\left[#1\right]\!}
\newcommand{\lrnorm}[1]{\left\|#1\right\|}
\newcommand{\lrset}[1]{\left\{#1\right\}}
\newcommand{\lrabs}[1]{\left|#1\right|}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\renewcommand{\t}[1]{\smash{\tilde{#1}}}
\newcommand{\wt}[1]{\smash{\widetilde{#1}}}
\newcommand{\wh}[1]{\smash{\widehat{#1}}}
\renewcommand{\O}{O}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\OO}[1]{\O\lr{#1}}
\newcommand{\tO}{\wt{\O}}
\newcommand{\tTheta}{\wt{\Theta}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\lrbra{#1}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\tsum}{\sum\nolimits}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\ind}[1]{\mathbb{I}\!\lrset{#1}}
\newcommand{\non}{\nonumber}
\newcommand{\poly}{\mathrm{poly}}

% \newcommand{\tr}{^{\mathsmaller\top}}
\newcommand{\tr}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\st}{\star}
\renewcommand{\dag}{\dagger}

%\newcommand{\kl}[2]{\mathsf{D}_\mathrm{KL}(#1,#2)}
\newcommand{\tv}[2]{\mathsf{D}_{\mathrm{TV}}(#1,#2)}
\newcommand{\ent}{\mathsf{H}}
\newcommand{\info}{\mathsf{I}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ep}{\varepsilon}
%\newcommand{\eps}{\epsilon}
\newcommand{\sig}{\sigma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\lam}{\lambda}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}

\newcommand{\eqdef}{:=}
\newcommand{\eq}{~=~}
\renewcommand{\leq}{~\le~}
\renewcommand{\geq}{~\ge~}
\newcommand{\lt}{~<~}
\newcommand{\gt}{~>~}
\newcommand{\then}{\quad\Rightarrow\quad}

\let\oldtfrac\tfrac
\renewcommand{\tfrac}[2]{\smash{\oldtfrac{#1}{#2}}}


\let\nablaold\nabla
\renewcommand{\nabla}{\nablaold\mkern-2.5mu}
%\let\cdotold\cdot
%\renewcommand{\cdot}{\mkern-2.5mu\cdotold\mkern-2.5mu}
%\newcommand{\param}{\cdotold}


%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
\newcommand{\ten}[1]{\mathcal{#1}}
\newcommand{\frob}[1]{\|#1\|_2}
\newcommand{\p}[2]{\textrm{Pr}[ #1\in #2] }
\newcommand{\pe}[2]{\mathop{\textrm{Pr}}\limits_{#1}\left[#2\right] }
%\newcommand{\one}[1]{\mathds{1}[#1]}
\newcommand{\inp}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\beps}{\bm{\eps}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\RE}[3]{\E{#1}{\sup_{#2}#3}}
%\newcommand{\rc}[1]{R\left(#1\right)}

